Urban-StyleGAN: Learning to Generate and Manipulate Images of Urban Scenes

A promise of Generative Adversarial Networks (GANs) is to provide cheap photorealistic data for training and validating AI models in autonomous driving. Despite their huge success, their performance on complex images featuring multiple objects is understudied. While some frameworks produce high-quality street scenes with little to no control over the image content, others offer more control at the expense of high-quality generation. A common limitation of both approaches is the use of global latent codes for the whole image, which hinders the learning of independent object distributions. Motivated by SemanticStyleGAN (SSG), a recent work on latent space disentanglement in human face generation, we propose a novel framework, Urban-StyleGAN, for urban scene generation and manipulation. We find that a straightforward application of SSG leads to poor results because urban scenes are more complex than human faces. To provide a more compact yet disentangled latent representation, we develop a class grouping strategy wherein individual classes are grouped into super-classes. Moreover, we employ an unsupervised latent exploration algorithm in the $\mathcal{S}$-space of the generator and show that it is more efficient than the conventional $\mathcal{W}^{+}$-space in controlling the image content. Results on the Cityscapes and Mapillary datasets show the proposed approach achieves significantly more controllability and improved image quality than previous approaches on urban scenes and is on par with general-purpose non-controllable generative models (like StyleGAN2) in terms of quality.

==> Figures/figure_1_SP_comparison.tex <==
\begin{figure}[t!]
    \centering
    \begin{center}
    \includegraphics[width=0.8\linewidth]{Figures/Images/symposium_table_1.png}
    \end{center}
    \caption{Comparing Semantic Palette's class distribution manipulation with SSG native manipulations by interpolating, and with our method of extracting meaningful directions in the S-space}
    \label{fig:figure_1_sp_comparison}
    \vspace{-1em}
\end{figure}

==> Figures/figure_2_manipulation_ablation.tex <==
\begin{figure}[t!]
    \centering
    \begin{center}
    \includegraphics[width=0.8\linewidth]{Figures/Images/symposium_table_2.png}
    \end{center}
    \caption{Comparing our two methods of extracting directions either from W space or S space with extracting directions from StyleGAN's generator latent space. }
    \label{fig:figure_2_edits_ablation}
    \vspace{-1em}
\end{figure}

==> Figures/figure_3_cityscapes_edits.tex <==
\begin{figure}[t!]
    \centering
    \begin{center}
    \includegraphics[width=0.8\linewidth]{Figures/Images/symposium_table_3.png}
    \end{center}
    \caption{Applying three different edits to three different classes for Cityscapes using directions discovered when exploring the S-space using GANSpace.}
    \label{fig:figure_3_cityscapes_edits}
    \vspace{-1em}
\end{figure}

==> Figures/figure_4_mapillary_edits.tex <==
\begin{figure}[t!]
    \centering
    \begin{center}
    \includegraphics[width=0.8\linewidth]{Figures/Images/symposium_table_4.png}
    \end{center}
    \caption{Applying three different edits to three different classes for Mapillary using directions discovered when exploring the S-space using GANSpace. }
    \label{fig:figure_4_mapillary_edits}
    \vspace{-1em}
\end{figure}

==> Tables/urban_scene_benchmark.tex <==
\begin{table}[h!] \centering  

\begin{tabular}{ccc} 
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Cityscapes}  \\
& FID  $\downarrow$ & mIoU  $\uparrow$   \\
\hline  
SB-GAN~\cite{sbgan} & 62.97 &   \\
SP~\cite{palette} & 52.5 & 21  \\
\textbf{Ours} & \textbf{9.8} & \textbf{34} \\ 
\hline
\end{tabular}

\caption{Image Synthesis on Cityscapes and Mapillary, Resolution $256^2$.} \label{table:urban_benchmark} 
%\vspace{-1.5em} 
\end{table}

%& \textbf{10.68} &
